Unsupervised Pre-training for Biomedical Question Answering

We explore the suitability of unsupervised representation learning methods on biomedical text -- BioBERT, SciBERT, and BioSentVec -- for biomedical question answering. To further improve unsupervised representations for biomedical QA, we introduce a new pre-training task from unlabeled data designed to reason about biomedical entities in the context. Our pre-training method consists of corrupting a given context by randomly replacing some mention of a biomedical entity with a random entity mention and then querying the model with the correct entity mention in order to locate the corrupted part of the context. This de-noising task enables the model to learn good representations from abundant, unlabeled biomedical text that helps QA tasks and minimizes the train-test mismatch between the pre-training task and the downstream QA tasks by requiring the model to predict spans. Our experiments show that pre-training BioBERT on the proposed pre-training task significantly boosts performance and outperforms the previous best model from the 7th BioASQ Task 7b-Phase B challenge.

==> BioSentVector.tex <==
To improve the correctness of the model's prediction, we  BioSentVec proposed by \cite{Chen2018BioSentVecCS} to evaluate the answers generated by the BioBERT and SciBERT. BioSentVec is the the first open set of sentence embeddings and it is trained with over 30 million documents from both scholarly articles in PubMed and clinical notes in the MIMICIII Clinical Database. The empirical result shows BioSentVec can better extract the semantic comparing to the other sentence to vectors models (fastSent, Sent2Vec, etc).
\par
In case of Yes/No we tried using both the unsupervised and supervised approach. In unsupervised approach, the question and context were transformed into vectors and computed cosine similarity between the question and context vectors. The intuition is that in case of 'yes' the question and context have high similarity, while the 'no' instance should be less similar. So, A threshold was set to differentiate yes and no answers. In supervised approach, the question and context vectors were concatenated and fed into fully connected neural network.   
\par
In case of Factoid and List, the way we use the BioSentVec takes two steps. In the first step, we compute the vector embeddings for the possible answers and question, and then calculate the cosine similarity between the two vectors. The assumption to choose a better answer is to pick the answer that has the higher similarity score with the question. 

==> Unsupervised.tex <==
\par 
Obtaining training data for Question Answering (QA) is often time-consuming and expensive. Most of current existing QA datasets are only available for general domains. Leveraging the current limited BioMedical annotated training corpus becomes a key point to improve the model's performance. In our work, we use the unsupervised data generation approach by taking the cloze translation proposed by \cite{lewis-etal-2019-unsupervised} to generated more data in Biomedical domain. 

\par 
The assumption is to have more data during the initial finetuning stages which contains more named entities of the specific domain even though the data is not of higher quality grammatically and semantically. In later stages of finetuning, high quality human annotated datasets such BioASQ and PubmedQA is used. Hence, we explore the idea on to what extent high quality training data is actually required and can benefit for Extractive QA. We implement this idea using the model published by Facebook \cite{lewis-etal-2019-unsupervised}.


% Our assumption is that in the initial finetuning epochs, the model learns about the field of data, name entities it has read and trained on, rather than the question and answer sounds or grammar. The backbone of unsupervised cloze translation model is showed in the figure\ref{fig:cloze}.


% \begin{figure}[h]
% \centering
% \includegraphics[width=\textwidth]{Figures/unsupervised.png}
%  \caption{ A schematic of cloze translation approach}
%  \label{fig:cloze}
% \end{figure}

\par 
% The Figure \ref{fig:cloze} shows the 
Three major components of the unsupervised model is used to generate more training data. First, the answer extractor will detect the name entity and noun phrase from the context and put a ``BLANKSPACE" mask on it. After this step, a cloze type question can be generated. The theory of this transformation is the name entity or the noun phrase will normally provide a definition or a specific object, which QA model needs to learn. After getting the cloze type question, based on the different name entity and noun phrase that were masked, different question type words(Where, When, How, What, Wh**) will be chosen to concatenate with the cloze question. For an example, if the noun phrase is a number (eg : ``2020"), the question type words is most likely to be ``When". After the concatenation, the pre-trained seq2seq QA model will be used to further transform the cloze type question to a new question, and therefore obtain syntactically meaningful question. By pairing the noun phrase as the answer and the newly generated question, the model forms the $<$question, answer$>$ pair to expand the current existing training corpus. 
